DiffPuter: Empowering Diffusion Models for Missing Data Imputation

Generative models play an important role in missing data imputation in that they aim to learn the joint distribution of full data. However, applying advanced deep generative models (such as Diffusion models) to missing data imputation is challenging due to 1) the inherent incompleteness of the training data and 2) the difficulty in performing conditional inference from unconditional generative models. To deal with these challenges, this paper introduces DiffPuter, a tailored diffusion model combined with the Expectation-Maximization (EM) algorithm for missing data imputation. DiffPuter iteratively trains a diffusion model to learn the joint distribution of missing and observed data and performs an accurate conditional sampling to update the missing values using a tailored reversed sampling strategy. Our theoretical analysis shows that DiffPuter's training step corresponds to the maximum likelihood estimation of data density (M-step), and its sampling step represents the Expected A Posteriori estimation of missing values (E-step). Extensive experiments across ten diverse datasets and comparisons with 17 different imputation methods demonstrate DiffPuter's superior performance. Notably, DiffPuter achieves an average improvement of 6.94% in MAE and 4.78% in RMSE compared to the most competitive existing method.

==> Tables/mcar_missing.tex <==
\begin{table}[h] 
    \centering
    \caption{MCAR, Missing 50\% MAE.} 
    \label{tbl:mcar-in-sample-acc}
    \small
    \begin{threeparttable}
    {
    \resizebox{\columnwidth}{!}
    % \scalebox{0.9}
    {
	\begin{tabular}{llcccccccccc}
            % \toprule[0.8pt]
            & \textbf{Method} &  \textbf{California} & \textbf{Letter} \textbf{Gesture } & \textbf{Magic} & \textbf{Bean} & \textbf{Adult} &  \textbf{Default} & \textbf{Shoppers} & \textbf{News} & \textbf{Beijing} \\
            \midrule[1.2pt] 
            \multicolumn{2}{l}{\hspace{-.5em} \textit{Traditional iterative}} \\
            & EM & $61.27${\tiny$\pm 0.12$} & $57.80${\tiny$\pm 0.22$} & $50.94${\tiny$\pm 0.27$} & $39.37${\tiny$\pm 0.06$} & $17.75${\tiny$\pm 0.18$} & $45.42$\\
            & MICE & $50.31${\tiny$\pm 0.21$} & $51.88${\tiny$\pm 0.30$} & $43.43${\tiny$\pm 0.19$} & $30.05${\tiny$\pm 1.17$} & $14.89${\tiny$\pm 0.90$} & $38.11$ &  {16} \\
            & MIRACLE & $62.28${\tiny$\pm 0.21$} & $55.79${\tiny$\pm 1.52$} & $45.74${\tiny$\pm 0.69$} & $39.33${\tiny$\pm 0.27$} & $20.88${\tiny$\pm 0.58$} & $44.61$ &  {12} \\
            & SoftImpute & $56.18${\tiny$\pm 0.08$} & $56.01${\tiny$\pm 0.07$} & $50.94${\tiny$\pm 0.27$} & $18.70${\tiny$\pm 0.05$} & $17.19${\tiny$\pm 0.07$} & $39.80$ &  {14} \\
            & MissForest & $63.51${\tiny$\pm 0.31$} & $56.97${\tiny$\pm 0.23$} & $51.10${\tiny$\pm 0.61$} & $37.55${\tiny$\pm 0.84$} & $19.13${\tiny$\pm 0.21$} & $45.65$  &  {9}\\
            \midrule
            \multicolumn{2}{l}{\hspace{-.5em} \textit{Dist. match}} \\
            & MOT & $63.85${\tiny$\pm 0.16$} & $71.95${\tiny$\pm 0.06$} & $56.91${\tiny$\pm 0.11$} & $38.62${\tiny$\pm 0.20$} & $19.51${\tiny$\pm 0.08$} & $50.16$ &  {5} \\
            & TDM & $62.64${\tiny$\pm 1.36$} & $63.41${\tiny$\pm 7.16$} & $55.00${\tiny$\pm 0.46$} & $30.62${\tiny$\pm 1.22$} & $19.38${\tiny$\pm 0.47$} & $46.21$ &  {8} \\
            \midrule
            \multicolumn{2}{l}{\hspace{-.5em} \textit{GNN}} \\
            & GRAPE & $69.84${\tiny$\pm 0.25$} & $73.85${\tiny$\pm 0.01$} & $57.32${\tiny$\pm 0.15$} & $40.83${\tiny$\pm 0.44$} & $19.92${\tiny$\pm 0.40$} & $52.35$ &  {4} \\
            & IGRM & $69.21${\tiny$\pm 0.29$} & OOM & $57.45${\tiny$\pm 0.16$} & OOM &  OOM & - & - \\
            \midrule
            % \multicolumn{2}{l}{\hspace{-.5em}
            % \textit{Predictive}} \\
            % & Remasker~\citep{remasker} & $69.18${\tiny$\pm 0.08$} & $76.88${\tiny$\pm 0.62$} & $57.86${\tiny$\pm 0.09$} & $44.33${\tiny$\pm 0.08$} & $\textbf{27.32}${\tiny$\pm 0.16$} & $51.60$ \\
            % \midrule
            \multicolumn{2}{l}{\hspace{-.5em} \textit{Generative models}} \\
            & MIWAE & $51.33${\tiny$\pm 0.08$} & $48.11${\tiny$\pm 0.02$} & $49.23${\tiny$\pm 0.61$} & $17.32${\tiny$\pm 0.01$} & $13.31${\tiny$\pm 0.28$} & $35.86$ &  {18} \\
            & GAIN & $53.73${\tiny$\pm 0.38$} & $54.49${\tiny$\pm 1.80$} & $47.25${\tiny$\pm 0.95$} & $34.20${\tiny$\pm 0.06$} & $14.71${\tiny$\pm 0.22$} & $40.88$ &  {13} \\
            & MCFlow & $60.31${\tiny$\pm 0.18$} & $68.36${\tiny$\pm 0..9$} & $52.73${\tiny$\pm 0.29$} & $30.08${\tiny$\pm 3.01$} & $15.84${\tiny$\pm 0.19$} & $45.46$ &  {11} \\      
            & TabCSDI & $58.72${\tiny$\pm 0.25$} & $50.57${\tiny$\pm 0.02$} & $43.24${\tiny$\pm 0.05$} & $17.49${\tiny$\pm 0.14$} & $13.03${\tiny$\pm 0.08$} & $36.61$ &  {17} \\
            & MissDiff & $57.39${\tiny$\pm 7.34$} & $66.01${\tiny$\pm 1.88$} & $48.10${\tiny$\pm 1.86$} & $41.39${\tiny$\pm 0.59$} & $19.02${\tiny$\pm 0.05$} & $46.38$ &  {7} \\
            \midrule
            \multicolumn{2}{l}{\hspace{-.5em}
            \textit{Other}} \\
            & KNN & $63.28${\tiny$\pm 0.52$} & $71.64${\tiny$\pm 0.34$} & $53.93${\tiny$\pm 0.28$} & $38.59${\tiny$\pm 0.17$} & $18.40${\tiny$\pm 0.39$} & $49.17$ &  {6} \\
            & Remasker & $69.18${\tiny$\pm 0.08$} & $76.88${\tiny$\pm 0.62$} & $57.86${\tiny$\pm 0.09$} & $44.33${\tiny$\pm 0.08$} & $\textbf{27.32}${\tiny$\pm 0.16$} &  $55.11$ &  {2} \\
            & HyperImpute & $64.99${\tiny$\pm 0.06$} & $74.39${\tiny$\pm 2.07$} & $\textbf{59.19}${\tiny$\pm 0.04$} & $40.29${\tiny$\pm 0.96$} & $26.91${\tiny$\pm 0.03$} & $53.15$ &  {3} \\
            \cmidrule{2-11}
            & \modelname & \\
		\end{tabular}
              }
              }

	\end{threeparttable}

\end{table}

\begin{table}[h] 
    \centering
    \caption{MCAR, missing 50\% RMSE.} 
    \label{tbl:mcar-in-sample-acc}
    \small
    \begin{threeparttable}
    {
    \resizebox{\columnwidth}{!}
    % \scalebox{0.9}
    {
	\begin{tabular}{llcccccccccc}
            % \toprule[0.8pt]
            & \textbf{Method} &  \textbf{California} & \textbf{Letter} \textbf{Gesture } & \textbf{Magic} & \textbf{Bean} & \textbf{Adult} &  \textbf{Default} & \textbf{Shoppers} & \textbf{News} & \textbf{Beijing} \\
            \midrule[1.2pt] 
            \multicolumn{2}{l}{\hspace{-.5em} \textit{Traditional iterative}} \\
            & EM & $61.27${\tiny$\pm 0.12$} & $57.80${\tiny$\pm 0.22$} & $50.94${\tiny$\pm 0.27$} & $39.37${\tiny$\pm 0.06$} & $17.75${\tiny$\pm 0.18$} & $45.42$\\
            & MICE & $50.31${\tiny$\pm 0.21$} & $51.88${\tiny$\pm 0.30$} & $43.43${\tiny$\pm 0.19$} & $30.05${\tiny$\pm 1.17$} & $14.89${\tiny$\pm 0.90$} & $38.11$ &  {16} \\
            & MIRACLE & $62.28${\tiny$\pm 0.21$} & $55.79${\tiny$\pm 1.52$} & $45.74${\tiny$\pm 0.69$} & $39.33${\tiny$\pm 0.27$} & $20.88${\tiny$\pm 0.58$} & $44.61$ &  {12} \\
            & SoftImpute & $56.18${\tiny$\pm 0.08$} & $56.01${\tiny$\pm 0.07$} & $50.94${\tiny$\pm 0.27$} & $18.70${\tiny$\pm 0.05$} & $17.19${\tiny$\pm 0.07$} & $39.80$ &  {14} \\
            & MissForest & $63.51${\tiny$\pm 0.31$} & $56.97${\tiny$\pm 0.23$} & $51.10${\tiny$\pm 0.61$} & $37.55${\tiny$\pm 0.84$} & $19.13${\tiny$\pm 0.21$} & $45.65$  &  {9}\\
            \midrule
            \multicolumn{2}{l}{\hspace{-.5em} \textit{Dist. match}} \\
            & MOT & $63.85${\tiny$\pm 0.16$} & $71.95${\tiny$\pm 0.06$} & $56.91${\tiny$\pm 0.11$} & $38.62${\tiny$\pm 0.20$} & $19.51${\tiny$\pm 0.08$} & $50.16$ &  {5} \\
            & TDM & $62.64${\tiny$\pm 1.36$} & $63.41${\tiny$\pm 7.16$} & $55.00${\tiny$\pm 0.46$} & $30.62${\tiny$\pm 1.22$} & $19.38${\tiny$\pm 0.47$} & $46.21$ &  {8} \\
            \midrule
            \multicolumn{2}{l}{\hspace{-.5em} \textit{GNN}} \\
            & GRAPE & $69.84${\tiny$\pm 0.25$} & $73.85${\tiny$\pm 0.01$} & $57.32${\tiny$\pm 0.15$} & $40.83${\tiny$\pm 0.44$} & $19.92${\tiny$\pm 0.40$} & $52.35$ &  {4} \\
            & IGRM & $69.21${\tiny$\pm 0.29$} & OOM & $57.45${\tiny$\pm 0.16$} & OOM &  OOM & - & - \\
            \midrule
            % \multicolumn{2}{l}{\hspace{-.5em}
            % \textit{Predictive}} \\
            % & Remasker~\citep{remasker} & $69.18${\tiny$\pm 0.08$} & $76.88${\tiny$\pm 0.62$} & $57.86${\tiny$\pm 0.09$} & $44.33${\tiny$\pm 0.08$} & $\textbf{27.32}${\tiny$\pm 0.16$} & $51.60$ \\
            % \midrule
            \multicolumn{2}{l}{\hspace{-.5em} \textit{Generative models}} \\
            & MIWAE & $51.33${\tiny$\pm 0.08$} & $48.11${\tiny$\pm 0.02$} & $49.23${\tiny$\pm 0.61$} & $17.32${\tiny$\pm 0.01$} & $13.31${\tiny$\pm 0.28$} & $35.86$ &  {18} \\
            & GAIN & $53.73${\tiny$\pm 0.38$} & $54.49${\tiny$\pm 1.80$} & $47.25${\tiny$\pm 0.95$} & $34.20${\tiny$\pm 0.06$} & $14.71${\tiny$\pm 0.22$} & $40.88$ &  {13} \\
            & MCFlow & $60.31${\tiny$\pm 0.18$} & $68.36${\tiny$\pm 0..9$} & $52.73${\tiny$\pm 0.29$} & $30.08${\tiny$\pm 3.01$} & $15.84${\tiny$\pm 0.19$} & $45.46$ &  {11} \\      
            & TabCSDI & $58.72${\tiny$\pm 0.25$} & $50.57${\tiny$\pm 0.02$} & $43.24${\tiny$\pm 0.05$} & $17.49${\tiny$\pm 0.14$} & $13.03${\tiny$\pm 0.08$} & $36.61$ &  {17} \\
            & MissDiff & $57.39${\tiny$\pm 7.34$} & $66.01${\tiny$\pm 1.88$} & $48.10${\tiny$\pm 1.86$} & $41.39${\tiny$\pm 0.59$} & $19.02${\tiny$\pm 0.05$} & $46.38$ &  {7} \\
            \midrule
            \multicolumn{2}{l}{\hspace{-.5em}
            \textit{Other}} \\
            & KNN & $63.28${\tiny$\pm 0.52$} & $71.64${\tiny$\pm 0.34$} & $53.93${\tiny$\pm 0.28$} & $38.59${\tiny$\pm 0.17$} & $18.40${\tiny$\pm 0.39$} & $49.17$ &  {6} \\
            & Remasker & $69.18${\tiny$\pm 0.08$} & $76.88${\tiny$\pm 0.62$} & $57.86${\tiny$\pm 0.09$} & $44.33${\tiny$\pm 0.08$} & $\textbf{27.32}${\tiny$\pm 0.16$} &  $55.11$ &  {2} \\
            & HyperImpute & $64.99${\tiny$\pm 0.06$} & $74.39${\tiny$\pm 2.07$} & $\textbf{59.19}${\tiny$\pm 0.04$} & $40.29${\tiny$\pm 0.96$} & $26.91${\tiny$\pm 0.03$} & $53.15$ &  {3} \\
            \cmidrule{2-11}
            & \modelname & \\
		\end{tabular}
              }
              }

	\end{threeparttable}

\end{table}

\begin{table}[h] 
    \centering
    \caption{MCAR, RMSE Missing 50\%.} 
    \label{tbl:mcar-in-sample-acc}
    \small
    \begin{threeparttable}
    {
    \resizebox{\columnwidth}{!}
    % \scalebox{0.9}
    {
	\begin{tabular}{llcccccccccc}
            % \toprule[0.8pt]
            & \textbf{Method} &  \textbf{California} & \textbf{Letter} \textbf{Gesture } & \textbf{Magic} & \textbf{Bean} & \textbf{Adult} &  \textbf{Default} & \textbf{Shoppers} & \textbf{News} & \textbf{Beijing} \\
            \midrule[1.2pt] 
            \multicolumn{2}{l}{\hspace{-.5em} \textit{Traditional iterative}} \\
            & EM & $61.27${\tiny$\pm 0.12$} & $57.80${\tiny$\pm 0.22$} & $50.94${\tiny$\pm 0.27$} & $39.37${\tiny$\pm 0.06$} & $17.75${\tiny$\pm 0.18$} & $45.42$\\
            & MICE & $50.31${\tiny$\pm 0.21$} & $51.88${\tiny$\pm 0.30$} & $43.43${\tiny$\pm 0.19$} & $30.05${\tiny$\pm 1.17$} & $14.89${\tiny$\pm 0.90$} & $38.11$ &  {16} \\
            & MIRACLE & $62.28${\tiny$\pm 0.21$} & $55.79${\tiny$\pm 1.52$} & $45.74${\tiny$\pm 0.69$} & $39.33${\tiny$\pm 0.27$} & $20.88${\tiny$\pm 0.58$} & $44.61$ &  {12} \\
            & SoftImpute & $56.18${\tiny$\pm 0.08$} & $56.01${\tiny$\pm 0.07$} & $50.94${\tiny$\pm 0.27$} & $18.70${\tiny$\pm 0.05$} & $17.19${\tiny$\pm 0.07$} & $39.80$ &  {14} \\
            & MissForest & $63.51${\tiny$\pm 0.31$} & $56.97${\tiny$\pm 0.23$} & $51.10${\tiny$\pm 0.61$} & $37.55${\tiny$\pm 0.84$} & $19.13${\tiny$\pm 0.21$} & $45.65$  &  {9}\\
            \midrule
            \multicolumn{2}{l}{\hspace{-.5em} \textit{Dist. match}} \\
            & MOT & $63.85${\tiny$\pm 0.16$} & $71.95${\tiny$\pm 0.06$} & $56.91${\tiny$\pm 0.11$} & $38.62${\tiny$\pm 0.20$} & $19.51${\tiny$\pm 0.08$} & $50.16$ &  {5} \\
            & TDM & $62.64${\tiny$\pm 1.36$} & $63.41${\tiny$\pm 7.16$} & $55.00${\tiny$\pm 0.46$} & $30.62${\tiny$\pm 1.22$} & $19.38${\tiny$\pm 0.47$} & $46.21$ &  {8} \\
            \midrule
            \multicolumn{2}{l}{\hspace{-.5em} \textit{GNN}} \\
            & GRAPE & $69.84${\tiny$\pm 0.25$} & $73.85${\tiny$\pm 0.01$} & $57.32${\tiny$\pm 0.15$} & $40.83${\tiny$\pm 0.44$} & $19.92${\tiny$\pm 0.40$} & $52.35$ &  {4} \\
            & IGRM & $69.21${\tiny$\pm 0.29$} & OOM & $57.45${\tiny$\pm 0.16$} & OOM &  OOM & - & - \\
            \midrule
            % \multicolumn{2}{l}{\hspace{-.5em}
            % \textit{Predictive}} \\
            % & Remasker~\citep{remasker} & $69.18${\tiny$\pm 0.08$} & $76.88${\tiny$\pm 0.62$} & $57.86${\tiny$\pm 0.09$} & $44.33${\tiny$\pm 0.08$} & $\textbf{27.32}${\tiny$\pm 0.16$} & $51.60$ \\
            % \midrule
            \multicolumn{2}{l}{\hspace{-.5em} \textit{Generative models}} \\
            & MIWAE & $51.33${\tiny$\pm 0.08$} & $48.11${\tiny$\pm 0.02$} & $49.23${\tiny$\pm 0.61$} & $17.32${\tiny$\pm 0.01$} & $13.31${\tiny$\pm 0.28$} & $35.86$ &  {18} \\
            & GAIN & $53.73${\tiny$\pm 0.38$} & $54.49${\tiny$\pm 1.80$} & $47.25${\tiny$\pm 0.95$} & $34.20${\tiny$\pm 0.06$} & $14.71${\tiny$\pm 0.22$} & $40.88$ &  {13} \\
            & MCFlow & $60.31${\tiny$\pm 0.18$} & $68.36${\tiny$\pm 0..9$} & $52.73${\tiny$\pm 0.29$} & $30.08${\tiny$\pm 3.01$} & $15.84${\tiny$\pm 0.19$} & $45.46$ &  {11} \\      
            & TabCSDI & $58.72${\tiny$\pm 0.25$} & $50.57${\tiny$\pm 0.02$} & $43.24${\tiny$\pm 0.05$} & $17.49${\tiny$\pm 0.14$} & $13.03${\tiny$\pm 0.08$} & $36.61$ &  {17} \\
            & MissDiff & $57.39${\tiny$\pm 7.34$} & $66.01${\tiny$\pm 1.88$} & $48.10${\tiny$\pm 1.86$} & $41.39${\tiny$\pm 0.59$} & $19.02${\tiny$\pm 0.05$} & $46.38$ &  {7} \\
            \midrule
            \multicolumn{2}{l}{\hspace{-.5em}
            \textit{Other}} \\
            & KNN & $63.28${\tiny$\pm 0.52$} & $71.64${\tiny$\pm 0.34$} & $53.93${\tiny$\pm 0.28$} & $38.59${\tiny$\pm 0.17$} & $18.40${\tiny$\pm 0.39$} & $49.17$ &  {6} \\
            & Remasker & $69.18${\tiny$\pm 0.08$} & $76.88${\tiny$\pm 0.62$} & $57.86${\tiny$\pm 0.09$} & $44.33${\tiny$\pm 0.08$} & $\textbf{27.32}${\tiny$\pm 0.16$} &  $55.11$ &  {2} \\
            & HyperImpute & $64.99${\tiny$\pm 0.06$} & $74.39${\tiny$\pm 2.07$} & $\textbf{59.19}${\tiny$\pm 0.04$} & $40.29${\tiny$\pm 0.96$} & $26.91${\tiny$\pm 0.03$} & $53.15$ &  {3} \\
            \cmidrule{2-11}
            & \modelname & \\
		\end{tabular}
              }
              }
	\end{threeparttable}
\end{table}


\begin{table}[h] 
    \centering
    \caption{MCAR, Missing 70\% MAE.} 
    \label{tbl:mcar-in-sample-acc}
    \small
    \begin{threeparttable}
    {
    \resizebox{\columnwidth}{!}
    % \scalebox{0.9}
    {
	\begin{tabular}{llcccccccccc}
            % \toprule[0.8pt]
            & \textbf{Method} &  \textbf{California} & \textbf{Letter} \textbf{Gesture } & \textbf{Magic} & \textbf{Bean} & \textbf{Adult} &  \textbf{Default} & \textbf{Shoppers} & \textbf{News} & \textbf{Beijing} \\
            \midrule[1.2pt] 
            \multicolumn{2}{l}{\hspace{-.5em} \textit{Traditional iterative}} \\
            & EM & $61.27${\tiny$\pm 0.12$} & $57.80${\tiny$\pm 0.22$} & $50.94${\tiny$\pm 0.27$} & $39.37${\tiny$\pm 0.06$} & $17.75${\tiny$\pm 0.18$} & $45.42$\\
            & MICE & $50.31${\tiny$\pm 0.21$} & $51.88${\tiny$\pm 0.30$} & $43.43${\tiny$\pm 0.19$} & $30.05${\tiny$\pm 1.17$} & $14.89${\tiny$\pm 0.90$} & $38.11$ &  {16} \\
            & MIRACLE & $62.28${\tiny$\pm 0.21$} & $55.79${\tiny$\pm 1.52$} & $45.74${\tiny$\pm 0.69$} & $39.33${\tiny$\pm 0.27$} & $20.88${\tiny$\pm 0.58$} & $44.61$ &  {12} \\
            & SoftImpute & $56.18${\tiny$\pm 0.08$} & $56.01${\tiny$\pm 0.07$} & $50.94${\tiny$\pm 0.27$} & $18.70${\tiny$\pm 0.05$} & $17.19${\tiny$\pm 0.07$} & $39.80$ &  {14} \\
            & MissForest & $63.51${\tiny$\pm 0.31$} & $56.97${\tiny$\pm 0.23$} & $51.10${\tiny$\pm 0.61$} & $37.55${\tiny$\pm 0.84$} & $19.13${\tiny$\pm 0.21$} & $45.65$  &  {9}\\
            \midrule
            \multicolumn{2}{l}{\hspace{-.5em} \textit{Dist. match}} \\
            & MOT & $63.85${\tiny$\pm 0.16$} & $71.95${\tiny$\pm 0.06$} & $56.91${\tiny$\pm 0.11$} & $38.62${\tiny$\pm 0.20$} & $19.51${\tiny$\pm 0.08$} & $50.16$ &  {5} \\
            & TDM & $62.64${\tiny$\pm 1.36$} & $63.41${\tiny$\pm 7.16$} & $55.00${\tiny$\pm 0.46$} & $30.62${\tiny$\pm 1.22$} & $19.38${\tiny$\pm 0.47$} & $46.21$ &  {8} \\
            \midrule
            \multicolumn{2}{l}{\hspace{-.5em} \textit{GNN}} \\
            & GRAPE & $69.84${\tiny$\pm 0.25$} & $73.85${\tiny$\pm 0.01$} & $57.32${\tiny$\pm 0.15$} & $40.83${\tiny$\pm 0.44$} & $19.92${\tiny$\pm 0.40$} & $52.35$ &  {4} \\
            & IGRM & $69.21${\tiny$\pm 0.29$} & OOM & $57.45${\tiny$\pm 0.16$} & OOM &  OOM & - & - \\
            \midrule
            % \multicolumn{2}{l}{\hspace{-.5em}
            % \textit{Predictive}} \\
            % & Remasker~\citep{remasker} & $69.18${\tiny$\pm 0.08$} & $76.88${\tiny$\pm 0.62$} & $57.86${\tiny$\pm 0.09$} & $44.33${\tiny$\pm 0.08$} & $\textbf{27.32}${\tiny$\pm 0.16$} & $51.60$ \\
            % \midrule
            \multicolumn{2}{l}{\hspace{-.5em} \textit{Generative models}} \\
            & MIWAE & $51.33${\tiny$\pm 0.08$} & $48.11${\tiny$\pm 0.02$} & $49.23${\tiny$\pm 0.61$} & $17.32${\tiny$\pm 0.01$} & $13.31${\tiny$\pm 0.28$} & $35.86$ &  {18} \\
            & GAIN & $53.73${\tiny$\pm 0.38$} & $54.49${\tiny$\pm 1.80$} & $47.25${\tiny$\pm 0.95$} & $34.20${\tiny$\pm 0.06$} & $14.71${\tiny$\pm 0.22$} & $40.88$ &  {13} \\
            & MCFlow & $60.31${\tiny$\pm 0.18$} & $68.36${\tiny$\pm 0..9$} & $52.73${\tiny$\pm 0.29$} & $30.08${\tiny$\pm 3.01$} & $15.84${\tiny$\pm 0.19$} & $45.46$ &  {11} \\      
            & TabCSDI & $58.72${\tiny$\pm 0.25$} & $50.57${\tiny$\pm 0.02$} & $43.24${\tiny$\pm 0.05$} & $17.49${\tiny$\pm 0.14$} & $13.03${\tiny$\pm 0.08$} & $36.61$ &  {17} \\
            & MissDiff & $57.39${\tiny$\pm 7.34$} & $66.01${\tiny$\pm 1.88$} & $48.10${\tiny$\pm 1.86$} & $41.39${\tiny$\pm 0.59$} & $19.02${\tiny$\pm 0.05$} & $46.38$ &  {7} \\
            \midrule
            \multicolumn{2}{l}{\hspace{-.5em}
            \textit{Other}} \\
            & KNN & $63.28${\tiny$\pm 0.52$} & $71.64${\tiny$\pm 0.34$} & $53.93${\tiny$\pm 0.28$} & $38.59${\tiny$\pm 0.17$} & $18.40${\tiny$\pm 0.39$} & $49.17$ &  {6} \\
            & Remasker & $69.18${\tiny$\pm 0.08$} & $76.88${\tiny$\pm 0.62$} & $57.86${\tiny$\pm 0.09$} & $44.33${\tiny$\pm 0.08$} & $\textbf{27.32}${\tiny$\pm 0.16$} &  $55.11$ &  {2} \\
            & HyperImpute & $64.99${\tiny$\pm 0.06$} & $74.39${\tiny$\pm 2.07$} & $\textbf{59.19}${\tiny$\pm 0.04$} & $40.29${\tiny$\pm 0.96$} & $26.91${\tiny$\pm 0.03$} & $53.15$ &  {3} \\
            \cmidrule{2-11}
            & \modelname & \\
		\end{tabular}
              }
              }

	\end{threeparttable}

\end{table}

\begin{table}[h] 
    \centering
    \caption{MCAR, missing 70\% RMSE.} 
    \label{tbl:mcar-in-sample-acc}
    \small
    \begin{threeparttable}
    {
    \resizebox{\columnwidth}{!}
    % \scalebox{0.9}
    {
	\begin{tabular}{llcccccccccc}
            % \toprule[0.8pt]
            & \textbf{Method} &  \textbf{California} & \textbf{Letter} \textbf{Gesture } & \textbf{Magic} & \textbf{Bean} & \textbf{Adult} &  \textbf{Default} & \textbf{Shoppers} & \textbf{News} & \textbf{Beijing} \\
            \midrule[1.2pt] 
            \multicolumn{2}{l}{\hspace{-.5em} \textit{Traditional iterative}} \\
            & EM & $61.27${\tiny$\pm 0.12$} & $57.80${\tiny$\pm 0.22$} & $50.94${\tiny$\pm 0.27$} & $39.37${\tiny$\pm 0.06$} & $17.75${\tiny$\pm 0.18$} & $45.42$\\
            & MICE & $50.31${\tiny$\pm 0.21$} & $51.88${\tiny$\pm 0.30$} & $43.43${\tiny$\pm 0.19$} & $30.05${\tiny$\pm 1.17$} & $14.89${\tiny$\pm 0.90$} & $38.11$ &  {16} \\
            & MIRACLE & $62.28${\tiny$\pm 0.21$} & $55.79${\tiny$\pm 1.52$} & $45.74${\tiny$\pm 0.69$} & $39.33${\tiny$\pm 0.27$} & $20.88${\tiny$\pm 0.58$} & $44.61$ &  {12} \\
            & SoftImpute & $56.18${\tiny$\pm 0.08$} & $56.01${\tiny$\pm 0.07$} & $50.94${\tiny$\pm 0.27$} & $18.70${\tiny$\pm 0.05$} & $17.19${\tiny$\pm 0.07$} & $39.80$ &  {14} \\
            & MissForest & $63.51${\tiny$\pm 0.31$} & $56.97${\tiny$\pm 0.23$} & $51.10${\tiny$\pm 0.61$} & $37.55${\tiny$\pm 0.84$} & $19.13${\tiny$\pm 0.21$} & $45.65$  &  {9}\\
            \midrule
            \multicolumn{2}{l}{\hspace{-.5em} \textit{Dist. match}} \\
            & MOT & $63.85${\tiny$\pm 0.16$} & $71.95${\tiny$\pm 0.06$} & $56.91${\tiny$\pm 0.11$} & $38.62${\tiny$\pm 0.20$} & $19.51${\tiny$\pm 0.08$} & $50.16$ &  {5} \\
            & TDM & $62.64${\tiny$\pm 1.36$} & $63.41${\tiny$\pm 7.16$} & $55.00${\tiny$\pm 0.46$} & $30.62${\tiny$\pm 1.22$} & $19.38${\tiny$\pm 0.47$} & $46.21$ &  {8} \\
            \midrule
            \multicolumn{2}{l}{\hspace{-.5em} \textit{GNN}} \\
            & GRAPE & $69.84${\tiny$\pm 0.25$} & $73.85${\tiny$\pm 0.01$} & $57.32${\tiny$\pm 0.15$} & $40.83${\tiny$\pm 0.44$} & $19.92${\tiny$\pm 0.40$} & $52.35$ &  {4} \\
            & IGRM & $69.21${\tiny$\pm 0.29$} & OOM & $57.45${\tiny$\pm 0.16$} & OOM &  OOM & - & - \\
            \midrule
            % \multicolumn{2}{l}{\hspace{-.5em}
            % \textit{Predictive}} \\
            % & Remasker~\citep{remasker} & $69.18${\tiny$\pm 0.08$} & $76.88${\tiny$\pm 0.62$} & $57.86${\tiny$\pm 0.09$} & $44.33${\tiny$\pm 0.08$} & $\textbf{27.32}${\tiny$\pm 0.16$} & $51.60$ \\
            % \midrule
            \multicolumn{2}{l}{\hspace{-.5em} \textit{Generative models}} \\
            & MIWAE & $51.33${\tiny$\pm 0.08$} & $48.11${\tiny$\pm 0.02$} & $49.23${\tiny$\pm 0.61$} & $17.32${\tiny$\pm 0.01$} & $13.31${\tiny$\pm 0.28$} & $35.86$ &  {18} \\
            & GAIN & $53.73${\tiny$\pm 0.38$} & $54.49${\tiny$\pm 1.80$} & $47.25${\tiny$\pm 0.95$} & $34.20${\tiny$\pm 0.06$} & $14.71${\tiny$\pm 0.22$} & $40.88$ &  {13} \\
            & MCFlow & $60.31${\tiny$\pm 0.18$} & $68.36${\tiny$\pm 0..9$} & $52.73${\tiny$\pm 0.29$} & $30.08${\tiny$\pm 3.01$} & $15.84${\tiny$\pm 0.19$} & $45.46$ &  {11} \\      
            & TabCSDI & $58.72${\tiny$\pm 0.25$} & $50.57${\tiny$\pm 0.02$} & $43.24${\tiny$\pm 0.05$} & $17.49${\tiny$\pm 0.14$} & $13.03${\tiny$\pm 0.08$} & $36.61$ &  {17} \\
            & MissDiff & $57.39${\tiny$\pm 7.34$} & $66.01${\tiny$\pm 1.88$} & $48.10${\tiny$\pm 1.86$} & $41.39${\tiny$\pm 0.59$} & $19.02${\tiny$\pm 0.05$} & $46.38$ &  {7} \\
            \midrule
            \multicolumn{2}{l}{\hspace{-.5em}
            \textit{Other}} \\
            & KNN & $63.28${\tiny$\pm 0.52$} & $71.64${\tiny$\pm 0.34$} & $53.93${\tiny$\pm 0.28$} & $38.59${\tiny$\pm 0.17$} & $18.40${\tiny$\pm 0.39$} & $49.17$ &  {6} \\
            & Remasker & $69.18${\tiny$\pm 0.08$} & $76.88${\tiny$\pm 0.62$} & $57.86${\tiny$\pm 0.09$} & $44.33${\tiny$\pm 0.08$} & $\textbf{27.32}${\tiny$\pm 0.16$} &  $55.11$ &  {2} \\
            & HyperImpute & $64.99${\tiny$\pm 0.06$} & $74.39${\tiny$\pm 2.07$} & $\textbf{59.19}${\tiny$\pm 0.04$} & $40.29${\tiny$\pm 0.96$} & $26.91${\tiny$\pm 0.03$} & $53.15$ &  {3} \\
            \cmidrule{2-11}
            & \modelname & \\
		\end{tabular}
              }
              }

	\end{threeparttable}

\end{table}

\begin{table}[h] 
    \centering
    \caption{MCAR, RMSE Missing 70\%.} 
    \label{tbl:mcar-in-sample-acc}
    \small
    \begin{threeparttable}
    {
    \resizebox{\columnwidth}{!}
    % \scalebox{0.9}
    {
	\begin{tabular}{llcccccccccc}
            % \toprule[0.8pt]
            & \textbf{Method} &  \textbf{California} & \textbf{Letter} \textbf{Gesture } & \textbf{Magic} & \textbf{Bean} & \textbf{Adult} &  \textbf{Default} & \textbf{Shoppers} & \textbf{News} & \textbf{Beijing} \\
            \midrule[1.2pt] 
            \multicolumn{2}{l}{\hspace{-.5em} \textit{Traditional iterative}} \\
            & EM & $61.27${\tiny$\pm 0.12$} & $57.80${\tiny$\pm 0.22$} & $50.94${\tiny$\pm 0.27$} & $39.37${\tiny$\pm 0.06$} & $17.75${\tiny$\pm 0.18$} & $45.42$\\
            & MICE & $50.31${\tiny$\pm 0.21$} & $51.88${\tiny$\pm 0.30$} & $43.43${\tiny$\pm 0.19$} & $30.05${\tiny$\pm 1.17$} & $14.89${\tiny$\pm 0.90$} & $38.11$ &  {16} \\
            & MIRACLE & $62.28${\tiny$\pm 0.21$} & $55.79${\tiny$\pm 1.52$} & $45.74${\tiny$\pm 0.69$} & $39.33${\tiny$\pm 0.27$} & $20.88${\tiny$\pm 0.58$} & $44.61$ &  {12} \\
            & SoftImpute & $56.18${\tiny$\pm 0.08$} & $56.01${\tiny$\pm 0.07$} & $50.94${\tiny$\pm 0.27$} & $18.70${\tiny$\pm 0.05$} & $17.19${\tiny$\pm 0.07$} & $39.80$ &  {14} \\
            & MissForest & $63.51${\tiny$\pm 0.31$} & $56.97${\tiny$\pm 0.23$} & $51.10${\tiny$\pm 0.61$} & $37.55${\tiny$\pm 0.84$} & $19.13${\tiny$\pm 0.21$} & $45.65$  &  {9}\\
            \midrule
            \multicolumn{2}{l}{\hspace{-.5em} \textit{Dist. match}} \\
            & MOT & $63.85${\tiny$\pm 0.16$} & $71.95${\tiny$\pm 0.06$} & $56.91${\tiny$\pm 0.11$} & $38.62${\tiny$\pm 0.20$} & $19.51${\tiny$\pm 0.08$} & $50.16$ &  {5} \\
            & TDM & $62.64${\tiny$\pm 1.36$} & $63.41${\tiny$\pm 7.16$} & $55.00${\tiny$\pm 0.46$} & $30.62${\tiny$\pm 1.22$} & $19.38${\tiny$\pm 0.47$} & $46.21$ &  {8} \\
            \midrule
            \multicolumn{2}{l}{\hspace{-.5em} \textit{GNN}} \\
            & GRAPE & $69.84${\tiny$\pm 0.25$} & $73.85${\tiny$\pm 0.01$} & $57.32${\tiny$\pm 0.15$} & $40.83${\tiny$\pm 0.44$} & $19.92${\tiny$\pm 0.40$} & $52.35$ &  {4} \\
            & IGRM & $69.21${\tiny$\pm 0.29$} & OOM & $57.45${\tiny$\pm 0.16$} & OOM &  OOM & - & - \\
            \midrule
            % \multicolumn{2}{l}{\hspace{-.5em}
            % \textit{Predictive}} \\
            % & Remasker~\citep{remasker} & $69.18${\tiny$\pm 0.08$} & $76.88${\tiny$\pm 0.62$} & $57.86${\tiny$\pm 0.09$} & $44.33${\tiny$\pm 0.08$} & $\textbf{27.32}${\tiny$\pm 0.16$} & $51.60$ \\
            % \midrule
            \multicolumn{2}{l}{\hspace{-.5em} \textit{Generative models}} \\
            & MIWAE & $51.33${\tiny$\pm 0.08$} & $48.11${\tiny$\pm 0.02$} & $49.23${\tiny$\pm 0.61$} & $17.32${\tiny$\pm 0.01$} & $13.31${\tiny$\pm 0.28$} & $35.86$ &  {18} \\
            & GAIN & $53.73${\tiny$\pm 0.38$} & $54.49${\tiny$\pm 1.80$} & $47.25${\tiny$\pm 0.95$} & $34.20${\tiny$\pm 0.06$} & $14.71${\tiny$\pm 0.22$} & $40.88$ &  {13} \\
            & MCFlow & $60.31${\tiny$\pm 0.18$} & $68.36${\tiny$\pm 0..9$} & $52.73${\tiny$\pm 0.29$} & $30.08${\tiny$\pm 3.01$} & $15.84${\tiny$\pm 0.19$} & $45.46$ &  {11} \\      
            & TabCSDI & $58.72${\tiny$\pm 0.25$} & $50.57${\tiny$\pm 0.02$} & $43.24${\tiny$\pm 0.05$} & $17.49${\tiny$\pm 0.14$} & $13.03${\tiny$\pm 0.08$} & $36.61$ &  {17} \\
            & MissDiff & $57.39${\tiny$\pm 7.34$} & $66.01${\tiny$\pm 1.88$} & $48.10${\tiny$\pm 1.86$} & $41.39${\tiny$\pm 0.59$} & $19.02${\tiny$\pm 0.05$} & $46.38$ &  {7} \\
            \midrule
            \multicolumn{2}{l}{\hspace{-.5em}
            \textit{Other}} \\
            & KNN & $63.28${\tiny$\pm 0.52$} & $71.64${\tiny$\pm 0.34$} & $53.93${\tiny$\pm 0.28$} & $38.59${\tiny$\pm 0.17$} & $18.40${\tiny$\pm 0.39$} & $49.17$ &  {6} \\
            & Remasker & $69.18${\tiny$\pm 0.08$} & $76.88${\tiny$\pm 0.62$} & $57.86${\tiny$\pm 0.09$} & $44.33${\tiny$\pm 0.08$} & $\textbf{27.32}${\tiny$\pm 0.16$} &  $55.11$ &  {2} \\
            & HyperImpute & $64.99${\tiny$\pm 0.06$} & $74.39${\tiny$\pm 2.07$} & $\textbf{59.19}${\tiny$\pm 0.04$} & $40.29${\tiny$\pm 0.96$} & $26.91${\tiny$\pm 0.03$} & $53.15$ &  {3} \\
            \cmidrule{2-11}
            & \modelname & \\
		\end{tabular}
              }
              }

	\end{threeparttable}

\end{table}

